Optimized Parallel Transmission in Elastic Optical Networks to Support High-Speed Ethernet

The need for optical parallelization is driven by the imminent optical capacity crunch, where the spectral efficiency required in the coming decades will be beyond the Shannon limit. To this end, the emerging high-speed Ethernet services at 100 Gbps, have already standardized options to utilize parallel optics to parallelize interfaces referred to as Multi-lane Distribution (MLD). OFDM-based optical network is a promising transmission option towards the goal of Ethernet parallelization. It can allocate optical resource tailored for a variety of bandwidth requirements and that in a fundamentally parallel fashion with each sub-carrier utilizing a frequency slot at a lower rate than if serial transmission was used. In this paper, we propose a novel parallel transmission framework designed for elastic (OFDM-based) optical networks to support high-speed Ethernet services, in-line with IEEE and ITU-T standards. We formulate an ILP optimization model based on integer linear programming, with consideration of various constraints, including spectrum fragmentation, differential delay and guard-band constraints. We also propose a heuristic algorithm which can be applied when the optimization model becomes intractable. The numerical results show the effectiveness and high suitability of elastic optical networks to support parallel transmission in high-speed Ethernet. To the best of our knowledge, this is the first attempt to investigate the parallel transmission in elastic optical networks to support standardized high-speed Ethernet.

==> literature.tex <==

@article{Winzer:2010,
 author = {Winzer, Peter J.},
 title = {Beyond 100G ethernet},
 journal = {IEEE Communication Magazine},
 volume = {48},
 number = {7},
 month = jul,
 year = {2010},
 issn = {0163-6804},
 pages = {26--30},
 numpages = {5},
 url = {http://dx.doi.org/10.1109/MCOM.2010.5496875},
 doi = {10.1109/MCOM.2010.5496875},
 acmid = {1840462},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
} 

@ARTICLE{Winzer:2012,
author={Winzer, P.J.},
journal={IEEE Photonics Journal},
title={Optical Networking Beyond WDM},
year={2012},
volume={4},
number={2},
pages={647-651},
}


@INPROCEEDINGS{Chralyvy:ecoc:2009,
author={Chralyvy, Andrew},
booktitle={35th European Conference on Optical Communication, 2009. ECOC '09},
title={Plenary paper: The coming capacity crunch},
%year={2009},
}



@misc{MEF,
title         = "Metro Ethernet Forum Technical Specifications",
howpublished  = "MEF Specifications ",
url = "http://metroethernetforum.org/",
}


@misc{cisco,
title = "Cisco SL-series",
 url="http://www.cisco.com/-en/US/products/hw/modules/ps2710/ps5479/index.html",
}


@article{Jinno:2009,
author={Jinno, M. and Takara, H. and Kozicki, B. and Tsukishima, Y. and Sone, Y. and Matsuoka, S.},
journal={IEEE Communications Magazine},
title={Spectrum-efficient and scalable elastic optical path network: architecture, benefits, and enabling technologies},
year={2009},
month={Nov.},
volume={47},
epages={66-73}, 
}

 

@ARTICLE{Jinno:2010,
author={Jinno, M. and Kozicki, B. and Takara, H. and Watanabe, A. and Sone, Y. and Tanaka, T. and Hirano, A.},
journal={IEEE Communications Magazine},
title={Distance-adaptive spectrum resource allocation in spectrum-sliced elastic optical path network},
year={2010},
month={Aug.},
volume={48},
number={8},
pages={138 -145}, 
}


@INPROCEEDINGS{Chen:infocom:2013,
author={Xiaomin Chen and Admela Jukan and Ashwin Gumaste},
booktitle={Mini Conference IEEE INFOCOM 2013},
title={Multipath De-fragmentation: Achieving Better Spectral Efficiency in Elastic Optical Path Networks},
year={2013},
month={April}
}

@INPROCEEDINGS{Chen:ICC:2013,
author={Xiaomin Chen and Yuesheng Zhong and Admela Jukan},
booktitle={IEEE ICC 2013},
title={Multipath Routing in Elastic Optical Networks with Distance-adaptive Modulation Formats},
year={2013},
month={June}

@INPROCEEDINGS{Kozicki:OFC:2009,
author={Kozicki, B. and Takara, H. and Yoshimatsu, T. and Yonenaga, K. and Jinno, M.},
booktitle={Proc. Conference on Optical Fiber Communication (OFC)},
title={Filtering characteristics of highly-spectrum efficient spectrum-sliced elastic optical path {(SLICE)} network},
year={2009},
month={Mar.},
volume={},
number={},
pages={1-3},
}

@INPROCEEDINGS{Sun:2008,
author={Yongmei Sun and Ono, T. and Takada, Atsushi and Tomizawa, M.},
booktitle={IEEE International Conference on Communications Workshops},
title={Wavelength-Group-Based Optical Virtual Concatenation Technique for Data-Intensive and Latency-Sensitive Applications},
year={2008},
pages={179-183},
 }


@INPROCEEDINGS{Shen:OFC:2011,
author={Gangxiang Shen and Qi Yang},
booktitle={ Proc. Conference on Optical Fiber Communication (OFC)},
title={From Coarse Grid to Mini-Grid to Gridless: How Much can Gridless Help Contentionless},
year={2011},
month={},
volume={},
number={},
pages={},
}




@article{Christo:JLT:2011,
author={Christodoulopoulos, K. and Tomkos, I. and Varvarigos, E.A.},
journal={IEEE/OSA Journal of Lightwave Technology},
title={Elastic Bandwidth Allocation in Flexible OFDM-Based Optical Networks},
year={2011},
month={May},
volume={29},
number={9},
pages={1354-1366},
}


@INPROCEEDINGS{Christo:Globecom:2010,
author={Christodoulopoulos, K. and Tomkos, I. and Varvarigos, E.A.},
booktitle={2010 IEEE Global Telecommunications Conference (GLOBECOM)},
title={Routing and Spectrum Allocation in OFDM-Based Optical Networks with Elastic Bandwidth Allocation},
year={2010},
month={Dec.},
volume={},
number={},
pages={1-6},
}


 
@article {Gumaste:Comag:2010,
author = "Ashwin Gumaste and Nalini Krishnaswamy",
title = " Proliferation of the optical transport network: A use case based study",
journal = "IEEE Communications Magazine",
year = "2010",
month ="Sept.",
volume = "48",
number = "9",
pages = "54-61",
}
 

@INPROCEEDINGS{Wang:infocom:2011,
author={Yang Wang and Xiaojun Cao and Yi Pan},
booktitle={Proc.{IEEE} INFOCOM,  },
title={A study of the routing and spectrum allocation in spectrum-sliced Elastic Optical Path networks},
year={2011},
month={Apr.},
volume={},
number={},
pages={1503-1511}, 
}

@INPROCEEDINGS{Takagi:OFC:2011,
author={Takagi, T. and Hasegawa, H. and Sato, K. and Sone, Y. and Kozicki, B. and Hirano, A. and Jinno, M.},
booktitle={Proc. OFC/NFOEC},
title={Dynamic routing and frequency slot assignment for elastic optical path networks that adopt distance adaptive modulation},
year={2011},
month={Mar.},
volume={},
number={},
pages={1-3}, 
}


@article {Shieh:2008,
author = "W. Shieh and H.Bao and Y.Tang",
title = "Coherent Optical OFDM: Theory and Design",
journal = "OSA Optics Express",
year = "2008",
month ="Jan.",
volume = "16",
number = "2",
pages = "841-859",
}
 
 
 

@INPROCEEDINGS{Patel:OFC:2011,
author={Ankitknmar N. Patel and  philip N. Ji and Jason P. Jue and Ting Wang},
booktitle={Proc. OFC/NFOEC},
title={Defragmentation of Transparent Flexible Optical {WDM (FWDM)} Networks},
year={2011},
month={},
volume={},
number={},
pages={1-3}, 
}



@ARTICLE{Klink:2009,
author={Klinkowski, M. and Walkowiak, K.},
journal={IEEE Communications Letters},
title={Routing and Spectrum Assignment in Spectrum Sliced Elastic Optical Path Network},
year={2011},
month={Aug.},
volume={15},
number={8},
pages={884-886}, 
}

 
 
@misc{ITU-T:G.709,
title         = "Interfaces for the Optical Transport Network {(OTN)}",
howpublished  = "ITU-T Recommendations ",
url = "http://www.itu.int/rec/T-REC-G.709/e",
}
 
 
@misc{Intel:datasheet,
title         = "Intel IXF19301 Datasheet", 
url = " http://www.intel.com/design/network/products/optical/tsp/IXF19301.htm",
}
 

@misc{SNDlib,
title         = "SNDlib", 
url = "http://sndlib.zib.de/home.action",
}  
 
@misc{gurobi,
title =  "Gurobi Optimizer",  
url = "http://www.gurobi.com/",
}

@INPROCEEDINGS{Huang:OFC:2007,
author={Sheng Huang and Rai, S. and Mukherjee, B.},
booktitle={OFC/NFOEC},
title={Survivable Differential Delay Aware Multi-Service Over SONET/SDH Networks with Virtual Concatenation},
year={2007},
month={Mar.},
volume={},
number={},
pages={1-3}, 
}



@inproceedings{Xu:2006,
 author = {Xu, W. and Rexford,J.},
 title = {{MIRO: Multi-path Interdomain ROtuing}},
 booktitle = {Proc.ACM SIGCOMM},
 year = {2006},
 month = {Sept.}
 pages={171-182},
}


 
@inproceedings{Sriva:ICC:2006,
author = {Srivastava,A. and Srivastava,A.},
title = {{Flow Aware Differential Delay Routing for Next-Generation Ethernet over SONET/SDH} },
booktitle = { Proc.{IEEE} ICC},
year = {2006},
pages={140-145},
} 
  
@inproceedings{Huang:Infocom:2008,
author={Huang, S. and Mukherjee, B. and Martel, C. },
title={Survivable Multipath Provisioning with Differential Delay Constraint in Telecom Mesh Networks},
booktitle ={ Proc.{IEEE}INFOCOM},
year={2008},
pages = {191-195}, 
}



@article{Demitra:2008,
 author = {Simeonidou, D. and others},
 title = {{Optical Network Services for Ultra High Definition Digital Media Distribution}},
 journal = {IEEE GOSP 2008, London, UK},
  %year = {2008},
 }
  

@inproceedings{Chen:CNSR:2009,
author = {Chen,X. and Chamania, M. and Jukan, A. and  Drummond,A. and  Fonseca,  N. L. S.},
title = {{On the Benefits of Multipath Routing for Distributed Data-intensive Applications with High Bandwidth Requirements and Multidomain Reach}},
booktitle = {IEEE Conference on Communication Networks and Services Research},
year = {2009},
month={may}  
 }

    
 

@electronic{Cisco:ECMP,
   title = {{BGP Multipath Load Sharing for Both eBGP and iBGP in an MPLS VPN}},
   url= {http://www.cisco.com},
}
 

@article{Chen:Globecom:2009,
 author = {Chen,X. and  Jukan,A. and  Drummond, A. C. and  Fonseca, N. L. S. da },
 title = {{A Multipath Routing Mechanism in Optical Networks with Extremely High Bandwidth Requests}},
 journal = {in Proc. IEEE GLOBECOM},
 year = {2009}
 }
 
 
@standard{802.3ba,
  title = "Carrier Sense Multiple Access with Collision Detection (CSMA/CD) Access method and Physical Layer Specifications",
  organization  = "IEEE",
  address       = "3 Park Avenue, NY",
  number        = "802.3ba",
  year          = "2010"
}

 
@ARTICLE{Chen:JOCN:2012,
author={Xiaomin Chen and Jukan, A.},
journal={Optical Communications and Networking, IEEE/OSA Journal of}, title={Optimized parallel transmission in OTN/WDM networks to support high-speed Ethernet with multiple lane distribution},
year={2012},
month={march },
volume={4},
number={3},
pages={248 -258},
keywords={Delay;High speed optical techniques;Optical buffering;Optical fiber networks;Optimization;Routing;WDM networks;IEEE standards;local area networks;wavelength division multiplexing;IEEE 802.3ba;OTN/WDM networks;bufferless parallel transmission;bufferless system design;computational complexity;electronic buffering;high speed Ethernet signal;integer linear programming problem;multiobjective evolutionary optimization;multiple lane distribution layer;optical channel;optical infrastructure;optical parallel transmission;optical transport network;optical virtual concatenation protocol;optimization framework;optimized parallel transmission;parallel transmission optimization;parallel wavelength routing;skew compensation;wavelength division multiplexing networks;Differential delay;High speed Ethernet;Parallel transmission;RWA;},
doi={10.1364/JOCN.4.000248},
ISSN={1943-0620},}



@ARTICLE{Zhu:JLT:2013,
author={Zuqing Zhu and Wei Lu and Liang Zhang and Ansari, N.},
journal={Journal of Lightwave Technology}, title={Dynamic Service Provisioning in Elastic Optical Networks With Hybrid Single-/Multi-Path Routing},
year={2013},
month={Jan},
volume={31},
number={1},
pages={15 -22},
}

@ARTICLE{Lu:Letter:2012,
author={Lu, Wei and Zhou, Xiang and Gong, Long and Zhang, Mingyang and Zhu, Zuqing},
journal={IEEE Communications Letters}, title={Dynamic Multi-Path Service Provisioning under Differential Delay Constraint in Elastic Optical Networks},
year={2013},
month={Jan.},
volume={17},
number={1},
pages={158 -161},
}
 
 
 
 @BOOK{Shieh:book,
   author = ",W. and Djordjevic, J.",
   title= "OFDM for Optical Communications",
   publisher = "Academic Press, Elsevier",
   year = "2010"
   }
 
 
 
 
 The BibTeX style designer's guide.
@electronic{IEEEexample:bibtexdesign,
  author        = "Oren Patashnik",
  title         = "Designing {{\BibTeX}} Styles",
  howpublished  = "{btxhak.pdf}",
  url           = "http://www.ctan.org/tex-archive/biblio/bibtex/contrib/doc/",
  month         = feb,
  year          = "1988"
}


A comprehensive BibTeX tutorial.
@electronic{IEEEexample:tamethebeast,
  author        = "Nicolas Markey",
  title         = "Tame the BeaST  ---  The B to X of {{\BibTeX}}",
  url           = "http://tug.ctan.org/tex-archive/info/bibtex/tamethebeast/",
  month         = oct,
  year          = "2005"
}


The BibTeX Tips and FAQ guide.
@electronic{IEEEexample:bibtexFAQ,
  author        = "David Hoadley and Michael Shell",
  title         = "{{\BibTeX}} Tips and {FAQ}",
  howpublished  = "{btxFAQ.pdf}",
  url           = "http://www.ctan.org/tex-archive/biblio/bibtex/contrib/doc/",
  month         = jan,
  year          = "2007"
}


The TeX FAQ
@electronic{IEEEexample:texfaq,
  author        = "Robin Fairbairns",
  title         = "The {{\TeX}} {FAQ}",
  url           = "http://www.tex.ac.uk/cgi-bin/texfaq2html/",
  month         = jan,
  year          = "2007"
}


A BibTeX Guide via Examples.
@electronic{IEEEexample:bibtexguide,
  author        = "Ki-Joo Kim",
  title         = "A {{\BibTeX}} Guide via Examples",
  howpublished  = "{bibtex\_guide.pdf}",
  url           = "http://www.geocities.com/kijoo2000/",
  month         = apr,
  year          = "2004"
}


TeX User Group Bibliography Archive
@electronic{IEEEexample:beebe_archive,
  author        = "Nelson H. F. Beebe",
  title         = "{{\TeX}} User Group Bibliography Archive",
  url           = "http://www.math.utah.edu:8080/pub/tex/bib/index-table.html",
  month         = aug,
  year          = "2006"
}

The natbib.sty package.
@electronic{ctan:natbib,
  author        = "Patrick W. Daly",
  title         = "The natbib.sty package",
  url           = "http://www.ctan.org/tex-archive/macros/latex/contrib/natbib/",
  month         = sep,
  year          = "2006"
}

The url.sty package.
@electronic{IEEEexample:urlsty,
  author        = "Donald Arseneau",
  title         = "The url.sty Package",
  url           = "http://www.ctan.org/tex-archive/macros/latex/contrib/misc/",
  month         = jun,
  year          = "2005",
}


The hyperref.sty package.
@electronic{IEEEexample:hyperrefsty,
  author        = "Sebastian Rahtz and Heiko Oberdiek",
  title         = "The hyperref.sty Package",
  url           = "http://www.ctan.org/tex-archive/macros/latex/contrib/hyperref/",
  month         = nov,
  year          = "2006",
}


